Audio-Visual Grouping Network for Sound Localization from Mixtures

Sound source localization is a typical and challenging task that predicts the location of sound sources in a video. Previous single-source methods mainly used the audio-visual association as clues to localize sounding objects in each image. Due to the mixed property of multiple sound sources in the original space, there exist rare multi-source approaches to localizing multiple sources simultaneously, except for one recent work using a contrastive random walk in the graph with images and separated sound as nodes. Despite their promising performance, they can only handle a fixed number of sources, and they cannot learn compact class-aware representations for individual sources. To alleviate this shortcoming, in this paper, we propose a novel audio-visual grouping network, namely AVGN, that can directly learn category-wise semantic features for each source from the input audio mixture and image to localize multiple sources simultaneously. Specifically, our AVGN leverages learnable audio-visual class tokens to aggregate class-aware source features. Then, the aggregated semantic features for each source can be used as guidance to localize the corresponding visual regions. Compared to existing multi-source methods, our new framework can localize a flexible number of sources and disentangle category-aware audio-visual representations for individual sound sources. We conduct extensive experiments on MUSIC, VGGSound-Instruments, and VGG-Sound Sources benchmarks. The results demonstrate that the proposed AVGN can achieve state-of-the-art sounding object localization performance on both single-source and multi-source scenarios. Code is available at \url{https://github.com/stoneMo/AVGN}.

==> SECTIONS/50_Ablation_Study/ab_vis_real.tex <==
\begin{figure}[t]
\centering
\fbox{\rule{0pt}{2in}
\rule{0.8\linewidth}{0pt}}
% \vspace{-3mm}
% \includegraphics[width=0.9\linewidth]{figs/figs_feat_cmp.pdf}
\caption{Real-world sound localization for off-screen and silent objects.}
\label{fig: exp_vis_real}
% \vspace{-5mm}
\end{figure}
 
